Regularizing Model Complexity and Label Structure for Multi-Label Text Classification

Multi-label text classification is a popular machine learning task where each document is assigned with multiple relevant labels. This task is challenging due to high dimensional features and correlated labels. Multi-label text classifiers need to be carefully regularized to prevent the severe over-fitting in the high dimensional space, and also need to take into account label dependencies in order to make accurate predictions under uncertainty. We demonstrate significant and practical improvement by carefully regularizing the model complexity during training phase, and also regularizing the label search space during prediction phase. Specifically, we regularize the classifier training using Elastic-net (L1+L2) penalty for reducing model complexity/size, and employ early stopping to prevent overfitting. At prediction time, we apply support inference to restrict the search space to label sets encountered in the training set, and F-optimizer GFM to make optimal predictions for the F1 metric. We show that although support inference only provides density estimations on existing label combinations, when combined with GFM predictor, the algorithm can output unseen label combinations. Taken collectively, our experiments show state of the art results on many benchmark datasets. Beyond performance and practical contributions, we make some interesting observations. Contrary to the prior belief, which deems support inference as purely an approximate inference procedure, we show that support inference acts as a strong regularizer on the label prediction structure. It allows the classifier to take into account label dependencies during prediction even if the classifiers had not modeled any label dependencies during training.

==> casestudy.tex <==
%!TEX root = ./body.tex
\section{Analysis of LSF}
From the results, we see that methods based on joint estimation (\textbf{CBM}, \textbf{CRF}, \textbf{PCC}) work better than method estimating $
p(||y||_1=s|x,y_l=1)$ directly (\textbf{LSF}). Theoretically, both approaches are consistent with F1 in the limit of infinite data and the \textbf{LSF} approach has the advantage of only requiring $L^2$ parameters compared with the joint estimation which requires $2^L$ parameters in the worst case. However, in practice, we find there are several reasons for which LSF does not perform well. OUr speculation is that directly predicting the number of relevant labels as in \textbf{LSF} is a very hard and unnatural formulation.  Each category here ("matching $s$ labels") does not have a fixed meaning, like "sport", "economy" in typical topical classification. ``matching 2 labels'' can mean many different things, such as matching "sky" and "cloud", or matching "dog" and "animal". So it is hard to establish a function for "matching 2 labels". This is especially hard for linear models like LR, in which probabilities are monotonic functions of scores, which in turn, are monotonic functions of features. 

==> table_feature.tex <==
\begin{table}[]
\centering
\caption{Feature Selected}
\vspace{0.1in}
\hspace{-3ex}
\resizebox{1.05\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{}         & {MEDICAL} & {BIBTEX} & {TMC} & {RCV1} &{BKMARK} 		&{SLASHD} & {OHSUM} \\
\textbf{features} & 1449             & 1836            & 49060           & 47236           & 2150           & 3125              & 12639            \\ \hline
\textbf{BR}       & 96               & 1836           & 46681            & 11838          &	2150	 	& 3002              & 2663             \\ \hline
\textbf{PS}       & 805              & 1836            & 46681            & 13843         & 2150  			& 3125              & 12639            \\ \hline
\textbf{PCC}      & 90               & 1836            & 2522             & 19146         & 2150 			& 2346              & 4627             \\ \hline
\textbf{CBM}      & 309              & 1836            & 46681            & 13759         & 2150 			& 3114              & 12639            \\ \hline
\textbf{LSF}      & 776              & 1836            & 46681            & 15246          &2150	 		& 3125              & 12516            \\ \hline
\textbf{CRF} & 1449           & 1836            & 49060          & 47236            &2150			& 3125            & 12639             \\ \hline
\end{tabular}
}
\label{table:feature}
\end{table}

==> table_main_result.tex <==
\begin{table}[h]
\centering
% \caption{Instance F1 with GFM}
\vspace{0.1in}
\resizebox{1.00\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
			& {MEDICAL} & {BIBTEX} & {TMC} & {RCV1} & {BKMARK} & {SLASHD}  & {OHSUM} \\ \hline
\textbf{BR}             & 78.07           & 41.04          & 62.72           & 73.18          & 25.54             & 50.37                & 62.03                 \\ \hline
\textbf{PS}             & 80.75           & 43.04          & 62.65           & \bf{76.26}     & -                 & 60.29                & 58.47                    \\ \hline
\textbf{PCC}            & 80.57           & 40.00          & 63.34           & 69.28          & -                 & 54.86                & 64.23                    \\ \hline
\textbf{CBM}            & \bf{84.65}      & \bf{49.87}     & 64.14           & 74.13          & 40.47         	  & \bf{65.28}           & \bf{70.24}                    \\ \hline
\textbf{LSF}            & 80.33           & 45.82          & 58.15           & 72.99          & 33.18             & 61.29                & 66.37                    \\ \hline
\textbf{CRF}            & 84.22           & 49.49          & \bf{64.65}      & 71.85          & \bf{41.69}        & 63.28                & 68.85                    \\ \hline
% \multicolumn{8}{l}{\textsuperscript{*}\footnotesize{All numbers are in percentages and \textbf{bold} refers the best performance for the dataset.}} \\
% \multicolumn{8}{l}{\textsuperscript{*}\footnotesize{"-": the corresponding method can't be finished by limited time/memory.}}
\end{tabular}
}
\caption{F-metric of different multi-label models + GFM prediction. All numbers are in percentages and \textbf{bold} refers the best performance for the dataset; "-": the corresponding method can't be finished by limited time/memory.}
% \vspace{1ex}
% \resizebox{1.05\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% 	 & {MEDICAL} & {BIBTEX} & {TMC} & {RCV1} & {BKMARK} & {SLASHD}  & {OHSUM} \\ \hline
% \textbf{BR}             & 77.71           & 39.77          & 58.61           & 72.56          & 23.06             & 50.04                & 54.92                 \\ \hline
% \textbf{PS}             & 80.54           & 40.35          & 60.22           & \bf{74.61}     & -                 & 55.72                & 59.17                    \\ \hline
% \textbf{PCC}            & 79.31           & 38.65          & 59.82           & 62.54          & -                 & 52.94                & 57.95                    \\ \hline
% \textbf{CBM}            & 82.79           & \bf{47.82}     & \bf{61.86}      & 73.63          & \bf{38.24}        & \bf{64.33}           & \bf{67.57}                    \\ \hline
% \textbf{CRF}            & \bf{84.30}      & 46.36          & 61.45           & 69.91          & 37.88             & 61.03                & 65.08                    \\ \hline
% % \multicolumn{8}{l}{\textsuperscript{*}\footnotesize{All numbers are in percentages and \textbf{bold} refers the best performance for the dataset.}} \\
% % \multicolumn{8}{l}{\textsuperscript{*}\footnotesize{"-": the corresponding method can't be finished by limited time/memory.}}
% \end{tabular}
% }
\label{table:mainResult}

\end{table}

==> table_main_result_noGFM.tex <==
\begin{table}[h]
\centering
% \caption{Instance F1 without GFM}
\resizebox{1.00\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
	 & {MEDICAL} & {BIBTEX} & {TMC} & {RCV1} & {BKMARKS} & {SLASHD}  & {OHSUM} \\ \hline
\textbf{BR}             & 77.71           & 39.77          & 58.61           & 72.56          & 23.06             & 50.04                & 54.92                 \\ \hline
\textbf{PS}             & 80.54           & 40.35          & 60.22           & \bf{74.61}     & -                 & 55.72                & 59.17                    \\ \hline
\textbf{PCC}            & 79.31           & 38.65          & 59.82           & 62.54          & -                 & 52.94                & 57.95                    \\ \hline
\textbf{CBM}            & 82.79           & \bf{47.82}     & \bf{61.86}      & 73.63          & \bf{38.24}        & \bf{64.33}           & \bf{67.57}                    \\ \hline
\textbf{CRF}            & \bf{84.30}      & 46.36          & 61.45           & 69.91          & 37.88             & 61.03                & 65.08                    \\ \hline
% \multicolumn{8}{l}{\textsuperscript{*}\footnotesize{All numbers are in percentages and \textbf{bold} refers the best performance for the dataset.}} \\
% \multicolumn{8}{l}{\textsuperscript{*}\footnotesize{"-": the corresponding method can't be finished by limited time/memory.}}
\end{tabular}
}
\label{table:mainResultWithoutGFM}
\caption{F-metric of different multi-label models + standard prediction. All numbers are in percentages and \textbf{bold} refers the best performance for the dataset; "-": the corresponding method can't be finished by limited time/memory.}
\end{table}

==> table_tune.tex <==
\begin{table*}[t]
\centering
% \caption{Tuned Hyper Parameters}
\vspace{0.1in}
 \resizebox{2.05\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{3}{|c|}{\textbf{}}                       & \multicolumn{3}{c|}{{MEDICAL}}     & \multicolumn{3}{c|}{{BIBTEX}}      & \multicolumn{3}{c|}{{TMC}}      & \multicolumn{3}{c|}{{RCV1}}    & \multicolumn{3}{c|}{{BKMARK}}        & \multicolumn{3}{c|}{{SLASHD}}    & \multicolumn{3}{c|}{{OHSUM}}     \\ \hline
\multicolumn{3}{|c|}{$v_{CRF}$}                       & \multicolumn{3}{c|}{$1$}                  & \multicolumn{3}{c|}{$2^{-2}$}             & \multicolumn{3}{c|}{$2^{-4}$}              & \multicolumn{3}{c|}{$1$}                & \multicolumn{3}{c|}{$2^{-4}$}                  & \multicolumn{3}{c|}{$2^2$}                & \multicolumn{3}{c|}{$1$}                  \\ \hline
$\lambda_{BR}$  & \multicolumn{2}{c|}{$\alpha_{BR}$}  & \multicolumn{2}{c|}{$10^{-3}$} & 1.0      & \multicolumn{2}{c|}{$10^{-5}$} & 1.0      & \multicolumn{2}{c|}{$10^{-3}$} & 0         & \multicolumn{2}{c|}{$10^{-7}$} & 0.8    & \multicolumn{2}{c|}{$10^{-7}$}       & 0.3     & \multicolumn{2}{c|}{$10^{-6}$} & 0.8      & \multicolumn{2}{c|}{$10^{-4}$} & 0.8      \\ \hline
$\lambda_{PS}$  & \multicolumn{2}{c|}{$\alpha_{PS}$}  & \multicolumn{2}{c|}{$10^{-4}$} & 0.6      & \multicolumn{2}{c|}{$10^{-6}$} & 0.4      & \multicolumn{2}{c|}{$10^{-3}$} & 0         & \multicolumn{2}{c|}{$10^{-7}$} & 0.8    & \multicolumn{2}{c|}{${10^{-7}}$} & ${0.3}$     & \multicolumn{2}{c|}{$10^{-4}$} & 0        & \multicolumn{2}{c|}{$10^{-6}$} & 0.1      \\ \hline
$\lambda_{PCC}$ & \multicolumn{2}{c|}{$\alpha_{PCC}$} & \multicolumn{2}{c|}{$10^{-3}$} & 1.0      & \multicolumn{2}{c|}{$10^{-5}$} & 1.0      & \multicolumn{2}{c|}{$10^{-4}$} & 1.0       & \multicolumn{2}{c|}{$10^{-4}$} & 0      & \multicolumn{2}{c|}{${10^{-7}}$} & ${0.3}$     & \multicolumn{2}{c|}{$10^{-4}$} & 0.9      & \multicolumn{2}{c|}{$10^{-4}$} & 0.5      \\ \hline
$\lambda_{LSF}$ & \multicolumn{2}{c|}{$\alpha_{LSF}$} & \multicolumn{2}{c|}{$10^{-5}$} & 0.9      & \multicolumn{2}{c|}{$10^{-4}$} & 0.2     & \multicolumn{2}{c|}{$10^{-3}$} & 0         & \multicolumn{2}{c|}{$10^{-5}$} & 0.5    & \multicolumn{2}{c|}{${10^{-7}}$} & ${0.3}$     & \multicolumn{2}{c|}{$10^{-3}$} & 0        & \multicolumn{2}{c|}{$10^{-4}$} & 0.1      \\ \hline
$\lambda_{CBM}$ & $\alpha_{CBM}$         & $K$        & $10^{-4}$         & 1.0        & 30       & $10^{-5}$         & 0.9        & 20       & $10^{-5}$          & 0         & 25        & ${10^{-7}}$      & ${0.8}$     & ${20}$     & ${10^{-7}}$         & ${0.3}$        & ${20}$      & $10^{-5}$         & 0.6        & 30       & $10^{-5}$         & 0.4        & 20       \\ \hline
\end{tabular}
 }
\caption {Tuned regularization parameters}
\label{table:tune}
\end{table*}


% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{}               & \textbf{medical} & \textbf{bibtex} & \textbf{tmc2007} & \textbf{rcv1v2} & \textbf{bookmarks} & \textbf{slashdot} & \textbf{ohsumed} \\ \hline
% $v_{CRF}$               & $1$              & $2^{-2}$        & $2^{-4}$         &    $1$          &  $2^{-4}$          &$2^2$              & $1$                  \\ \hline
% $\lambda/\alpha_{BR}$   &$10^{-3}/1.0$     &$10^{-5}/1.0$    &$10^{-3}/0$       & $10^{-7}/0.8$   & $10^{-7}/0.3$      &$10^{-6}/0.8$      &$10^{-4}/0.8$                  \\ \hline
% $\lambda/\alpha_{PS}$   &$10^{-4}/0.6$     &$10^{-6}/0.4$    &$10^{-3}/0$       & $10^{-7}/0.8$   & ${10^{-7}/0.3}$& $10^{-4}/0$       &$10^{-6}/0.1$     \\ \hline
% $\lambda/\alpha_{PCC}$  &$10^{-3}/1.0$     &$10^{-5}/1.0$    &$10^{-4}/1.0$     &$10^{-4}/0$      &${10^{-7}/0.3}$ &$10^{-4}/0.9$      &$10^{-4}/0.5$     \\ \hline
% $\lambda/\alpha_{LSF}$  &$10^{-5}/0.9$     &$10^{-4}/0.2$    &$10^{-3}/ 0$      &$10^{-5}/0.5$    &${10^{-7}/0.3}$ &$10^{-3}/0$        &$10^{-4}/0.1$     \\ \hline
% $\lambda/\alpha/K_{CBM}$&$10^{-4}/1.0/30$  &$10^{-5}/0.9/20$ &$10^{-5}/0/25$    &${10^{-7}/0.8/20}$ &${10^{-7}/0.3/20}$ &$10^{-5}/0.6/30$&$10^{-5}/0.4/20$  \\ \hline
% \end{tabular}



% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \textbf{dataset} & \textbf{$v_{CRF}$} & \textbf{$\lambda/\alpha_{BR}$} & \textbf{$\lambda/\alpha_{PS}$} &\textbf{$\lambda/\alpha_{PCC}$} &\textbf{$\lambda/\alpha_{LSF}$} & \textbf{$\lambda/\alpha/K_{CBM}$} \\ \hline
% medical          &  $1$               &  $10^{-3}/1.0$       & $10^{-4}/0.6$          &    $10^{-3}/1.0$     & $10^{-5}/0.9$        & $10^{-4}/1.0/30$                   \\ \hline
% bibtex           &  $2^{-2}$          &  $10^{-5}/1.0$       & $10^{-6}/0.4$          &    $10^{-5}/1.0$     & $10^{-4}/0.2$        & $10^{-5}/0.9/20$                   \\ \hline
% tmc2007          &  $2^{-4}$          &  $10^{-3}/0$         & $10^{-3}/0$            &    $10^{-4}/1.0$     & $10^{-3}/ 0$         & $10^{-5}/0/25$                      \\ \hline
% rcv1v2           &  $1$               &  $10^{-7}/0.8$       & $10^{-7}/0.8$          &    $10^{-4}/0$       & $10^{-5}/0.5$        & ${10^{-7}/0.8/20}$              \\ \hline
% bookmarks        &  $2^{-4}$          &  $10^{-7}/0.3$       & ${10^{-7}/0.3}$    &${10^{-7}/0.3}$   &${10^{-7}/0.3}$ & ${10^{-7}/0.3/20}$                \\ \hline
% slashdot     &  $2^2$             &  $10^{-6}/0.8$       & $10^{-4}/0$            &    $10^{-4}/0.9$     & $10^{-3}/0$          & $10^{-5}/0.6/30$                         \\ \hline
% ohsumed      &  $1$               &  $10^{-4}/0.8$       & $10^{-6}/0.1$          &    $10^{-4}/0.5$     & $10^{-4}/0.1$        & $10^{-5}/0.4/20$                         \\ \hline
% % \multicolumn{4}{l}{\textsuperscript{*}\footnotesize{\textbf{Bold} means it is hard to tune hyper parameters for the method on relative large dataset, it will use the tuned hyper parameters as the same as BR tuned.}}
% \end{tabular}

% \begin{table}[]
% \centering
% \caption{My caption}
% \label{my-label}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{3}{|c|}{\textbf{}}                       & \multicolumn{3}{c|}{\textbf{medical}}     & \multicolumn{3}{c|}{\textbf{bibtex}}      & \multicolumn{3}{c|}{\textbf{tmc2007}}            & \multicolumn{3}{c|}{\textbf{rcv1v2}}    & \multicolumn{3}{c|}{\textbf{bookmarks}}        & \multicolumn{3}{c|}{\textbf{slashdot}}    & \multicolumn{3}{c|}{\textbf{ohsumed}}     \\ \hline
% \multicolumn{3}{|c|}{$v_{CRF}$}                       & \multicolumn{3}{c|}{$1$}                  & \multicolumn{3}{c|}{$2^{-2}$}             & \multicolumn{3}{c|}{$2^{-4}$}                    & \multicolumn{3}{c|}{$1$}                & \multicolumn{3}{c|}{$2^{-4}$}                  & \multicolumn{3}{c|}{$2^2$}                & \multicolumn{3}{c|}{$1$}                  \\ \hline
% $\lambda_{BR}$  & \multicolumn{2}{c|}{$\alpha_{BR}$}  & \multicolumn{2}{c|}{$10^{-3}$} & 1.0      & \multicolumn{2}{c|}{$10^{-5}$} & 1.0      & \multicolumn{2}{c|}{$10^{-3}/0$}    &            & \multicolumn{2}{c|}{$10^{-7}$} & 0.8    & \multicolumn{2}{c|}{$10^{-7}$}       & 0.3     & \multicolumn{2}{c|}{$10^{-6}$} & 0.8      & \multicolumn{2}{c|}{$10^{-4}$} & 0.8      \\ \hline
% $\lambda_{PS}$  & \multicolumn{2}{c|}{$\alpha_{PS}$}  & \multicolumn{2}{c|}{$10^{-4}$} & 0.6      & \multicolumn{2}{c|}{$10^{-6}$} & 0.4      & \multicolumn{2}{c|}{$10^{-3}/0$}    &            & \multicolumn{2}{c|}{$10^{-7}$} & 0.8    & \multicolumn{2}{c|}{${10^{-7}}$} & 0.3     & \multicolumn{2}{c|}{$10^{-4}$} & 0        & \multicolumn{2}{c|}{$10^{-6}$} & 0.1      \\ \hline
% $\lambda_{PCC}$ & \multicolumn{2}{c|}{$\alpha_{PCC}$} & \multicolumn{2}{c|}{$10^{-3}$} & 1.0      & \multicolumn{2}{c|}{$10^{-5}$} & 1.0      & \multicolumn{2}{c|}{$10^{-4}/1.0$}  &            & \multicolumn{2}{c|}{$10^{-4}$} & 0      & \multicolumn{2}{c|}{${10^{-7}}$} & 0.3     & \multicolumn{2}{c|}{$10^{-4}$} & 0.9      & \multicolumn{2}{c|}{$10^{-4}$} & 0.5      \\ \hline
% $\lambda_{LSF}$ & \multicolumn{2}{c|}{$\alpha_{LSF}$} & \multicolumn{2}{c|}{$10^{-5}$} & 0.9      & \multicolumn{2}{c|}{$10^{-4}$} & /0.2     & \multicolumn{2}{c|}{$10^{-3}/ 0$}   &            & \multicolumn{2}{c|}{$10^{-5}$} & 0.5    & \multicolumn{2}{c|}{${10^{-7}}$} & 0.3     & \multicolumn{2}{c|}{$10^{-3}$} & 0        & \multicolumn{2}{c|}{$10^{-4}$} & 0.1      \\ \hline
% $\lambda_{CBM}$ & $\alpha_{CBM}$         & $K$        & $10^{-4}$         & 1.0        & 30       & $10^{-5}$         & 0.9        & 20       & \multicolumn{2}{c|}{$10^{-5}/0/25$} &            & ${10^{-7}}$      & 0.8     & 20     & ${10^{-7}}$         & 0.3        & 20      & $10^{-5}$         & 0.6        & 30       & $10^{-5}$         & 0.4        & 20       \\ \hline
% \end{tabular}
% \end{table}
